Situational Confidence Assistance for Lifelong Shared Autonomy

Shared autonomy enables robots to infer user intent and assist in accomplishing it. But when the user wants to do a new task that the robot does not know about, shared autonomy will hinder their performance by attempting to assist them with something that is not their intent. Our key idea is that the robot can detect when its repertoire of intents is insufficient to explain the user's input, and give them back control. This then enables the robot to observe unhindered task execution, learn the new intent behind it, and add it to this repertoire. We demonstrate with both a case study and a user study that our proposed method maintains good performance when the human's intent is in the robot's repertoire, outperforms prior shared autonomy approaches when it isn't, and successfully learns new skills, enabling efficient lifelong learning for confidence-based shared autonomy.

==> [ICRA'21][Zurek]Situational Confidence Shared Autonomy wbbl/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
%\adnote{much shorter background, no need for details about dragan vs javdani vs whatnot (reads like forced related work into the intro and distracts from the paper's point); goals/skills/intent consistency; representing intent generally via a reward function; more punchy introduction of the idea: enable robots to detect when they are missing an intent, learn it, add it to its repertoire -- right now its rather procedural}

%what is shared autonomy
%Shared autonomy \cite{aigner1997human,dragan2013blending,reddy2018shared,losey2018review,goertz1963manipulators,farraj2018hapticshared,losey2020latent,li2011dynamic,erdogan2017effect,brown2014balancing,crandall2017human} enables robots to assist human operators to more effectively accomplish what they want. Rather than directly executing the human's control input, a typical framework for shared autonomy has the robot estimate the human's intent and execute controls that help achieve it \cite{dragan2013blending,javdani2015shared,muelling2017autonomy,perez2015fast,reddy2018shared}.

In shared autonomy \cite{aigner1997human,dragan2013blending,reddy2018shared,losey2018review,goertz1963manipulators,farraj2018hapticshared,losey2020latent,li2011dynamic,erdogan2017effect,brown2014balancing,crandall2017human}, robots assist human operators to perform their objectives more effectively. Here, rather than directly executing the human's control input, a typical framework has the robot estimate the human's intent and execute controls that help achieve it \cite{dragan2013blending,javdani2015shared,muelling2017autonomy,perez2015fast,reddy2018shared}.

%whats is the problem 
%These methods perform well when the robot has access to a set of possible intents the human might have, e.g. the objects the human might want to reach, or the buttons they might want to push \cite{dragan2013blending,javdani2015shared}. But in reality, users of these systems will inevitably want to perform tasks that are outside the repertoire of known intents -- they might want to reach for a goal the robot does not know about, or perform a totally new task, like pouring their cup of water into the sink. This presents a three-fold challenge for shared autonomy. First, the robot will be unable to help with something it does not know about. Second, and perhaps more importantly, it will attempt to assist with whatever wrong intent it infers, interfering with what the user is trying to do and hindering their performance. This happens when the robot plans in expectation \cite{javdani2015shared}, and, as our experiments will demonstrate, it happens even when the robot arbitrates the amount of assistance based on its confidence in the most likely goal \cite{dragan2013blending}. Third, the 100th time the person attempts the new task, it will remain just as difficult as the first time.

These methods succeed when the robot knows the set of possible human intents a priori, e.g. the objects the human might want to reach, or the buttons they might want to push \cite{dragan2013blending,javdani2015shared}. But realistically, users of these systems will inevitably want to perform tasks outside the repertoire of known intents -- they might want to reach for a goal unknown to the robot, or perform a new task like pouring a cup of water into a sink. This presents a three-fold challenge for shared autonomy. First, the robot will be unable to recognize and help with something unknown. Second, and perhaps more importantly, it will attempt to assist with whatever wrong intent it infers, interfering with what the user is trying to do and hindering their performance. This happens when the robot plans in expectation \cite{javdani2015shared}, and, as our experiments will demonstrate, it happens even when the robot arbitrates the amount of assistance based on its confidence in the most likely goal \cite{dragan2013blending}. Third, the new task remains just as difficult as the first time even after arbitrarily many attempts.

Our key idea is that the robot should detect that the user is trying something new and give them control. This then presents an opportunity for the robot to observe the new executed trajectory, learn the underlying intent that explains it, and add it to its repertoire so that it can infer and assist for this intent in the future.

\begin{figure}[t]
\includegraphics[width=\linewidth]{figures/lifelong_assistance_trajs.png}
\centering
\caption{We propose an approach for lifelong shared autonomy that enables a robot to detect when its set of known human intents is insufficient to explain the current human behavior. Rather than trying to assist for the wrong intent, the robot learns from novel teleoperations to learn a model of the new intent, allowing for lifelong confidence-based assistance.}
\label{fig:front_fig}
\vspace*{-0.5cm}
\end{figure}

To achieve this, we need two ingredients: 1) a way for the robot to detect its repertoire of intents is insufficient, and 2) a representation of intents that enables learning new tasks throughout its lifetime, adding them to its repertoire, and performing inference over them in a unified way with the initial known intents. 
For the latter, we use cost functions to unify goals and general skills like pouring into the same representation.
This then enables the former: when the human acts too suboptimally for any of the known cost functions, it suggests the robot lacks the correct set of costs.

Our approach takes inspiration from recent work on hypothesis misspecification where the robot recognizes when its cost function features are insufficient to explain human demonstrations and corrections \cite{bobu2020quantifying}, and updates the cost in proportion to the \textit{situational confidence} in these features' ability to explain input. We extend detecting hypothesis mispecification to the context of shared autonomy, in which there are multiple intents, represented as cost functions, and the robot seeks to recognize whether any of the known intents explain the human input sufficiently. The robot can then arbitrate its assistance based on its confidence in the most likely intent being what the human wanted.

Our approach, which we call Confidence-Aware Shared Autonomy (CASA), allows the robot to ascertain whether the human inputs are associated with a known or new task. 
By arbitrating the user's input based on the confidence in the most likely intent, \algabbr follows a standard policy blending assistance approach if the task is known, and otherwise gives the user full control. Additionally, \algabbr allows the user to provide a few demonstrations of the new intent, which the robot uses to learn a cost function via Inverse Reinforcement Learning (IRL) \cite{finn2016guided} and add it to its set of intents. This enables lifelong shared autonomy, where the robot helps when it is confident in what the user wants and learns new intents when it detects that the human is doing something novel, so that it can assist with that intent in the future.

%\adnote{now you can have your description of what happens: if the task is known, we infer and assist; if it's not known,  direct control (or explain we arbitrate based on just how unexplained the human behavior is), get demonstrations, learn the new skill, add it in}

%\adnote{if space, you can recap the three benefits as you are doing in the penultimate par of your current intro}

%\adnote{avoid the enumeration of what happens in the paper from the last paragraph; replace it with "We test our approach in a user study .... the results suggest that (we're better for novel tasks, we maintain good performance on known tasks, we learn the new task)..."}

%Shared autonomy \cite{aigner1997human,dragan2013blending,reddy2018shared,losey2018review} allows robots to assist people in accomplishing tasks which may be difficult for the human to accomplish by themselves. 
%This is often done by adding or blending robot controls to the controls of the human operator. 
%As a common tool for facilitating human-robot teaming, it has been applied to many different domains, such as handling radioactive waste \cite{goertz1963manipulators,farraj2018hapticshared}, assisting users to eat or cook \cite{losey2020latent}, wheel chair navigation \cite{li2011dynamic,erdogan2017effect}, controlling robot swarms~\cite{brown2014balancing,crandall2017human}, rehabilitation \cite{losey2018review}, and quadrotor control \cite{reddy2018shared}.

%To be good at assisting humans, robots need to understand what the person is trying to do. Many shared autonomy frameworks assume that the human's intent is hidden from the robot, and rely on intent recognition followed by assistance based on the inferred intent \cite{dragan2013blending,javdani2015shared,muelling2017autonomy,perez2015fast,reddy2018shared}. However, these methods all assume that the human is attempting to accomplish one of several known skills or goals. This is problematic if the human is trying to do something novel since the ``assistance" might actually hinder the human. 


%Prior work has suggested a confidence-based policy blending approach that assists less if the robot is uncertain about the true human intent \cite{dragan2013blending}
%Prior work on shared control for teleoperation focuses on assisting a user to accomplish a task. 
%Common in shared control for teleoperation is for the robot to predict what the human is trying to do and then assist for that prediction.
%Dragan et al.~\cite{dragan2013blending} propose a policy blending approach where the robot first performs goal prediction then assists to one of a predetermined set of goals. The assistance is blended based on the confidence in the goal, giving more control to the user when the robot is more uncertain; however, as we show later, this method still attempts weak assistance towards the most likely goal out of the predefined goal set, hindering a human performing a novel task. 

%Javdani et al.~\cite{javdani2015shared} propose an alternative approach that maintains the posterior distribution over likely goals, and assists even when confidence for any goal is low. 
%However, they found that users prefer the policy-blending approach of Dragan et al.~\cite{dragan2013blending} to their proposed distribution-based assistance. We, thus, take inspiration from the policy blending formalism to shared autonomy \cite{dragan2013blending}, in which the executed robot control is a convex combination of the human's control and the robot's assistance. 

%We propose a novel shared autonomy approach, which we call \algname (\algabbr), that allows a robot to use a set of predefined goals, but recognize when the human is trying to do something novel. 
%Prior work on shared autonomy typically assumes the user is only trying to get to a target location or goal \cite{dragan2013blending,goertz1963manipulators,farraj2018hapticshared,aigner1997human,li2011dynamic,erdogan2017effect,javdani2015shared}. 
%In contrast, we propose a shared control framework that works will any kind of skill that is parameterized by a cost function. 
%Furthermore, to the best of our knowledge, we propose the first algorithm for lifelong shared autonomy where the robot not only assists a human when they perform known skills, but can recognize and learn novel skills, which are then added into its library of known skills for future use.

%In order to detect a novel intent, we extend recent work on hypothesis misspecification that seeks to recognize when a robot's cost function features are insufficient to explain human demonstrations and corrections \cite{bobu2020quantifying}. We extend hypothesis mispecification to the context of shared autonomy, in which there are multiple skills, represented as cost functions, and the robot seeks to recognize whether any of the known cost functions are sufficient to explain the human input. Given human input such as a human teleoperating a robot arm, our approach allows the robot to quickly ascertain whether the human inputs are associated with a known task or associated with some novel task. If the task is known, then \algabbr follows a standard policy blending approach to shared autonomy. However, if the task is novel, \algabbr gives full control to the user. Additionally, our proposed approach allows the user to give a small number of demonstrations of the new skill, which the robot uses to learn a cost function for the new skill via inverse reinforcement learning \cite{finn2016guided}. \algabbr then adds this cost function to its existing set of known skills. This enables a lifelong learning approach for shared autonomy, where the robot is constantly monitoring the human's inputs, helping when it is confident what the human wants, and learning new skills from the human when it detects that the human is doing something novel so that it can assist with that skill in the future.

%\algabbr has three main benefits: (1) it enhances task performance when the human performs a known intent, (2) it does not hinder task performance when the human performs a novel intent, and (3) it enables lifelong intent acquisition by learning from novel human actions and adding new intents to its set. Thus, \algabbr affords a virtuous cycle of intent learning and assistance: the robot's set of known intents improves over time, allowing the robot to assist the human over an increasingly wide range of tasks.

We test our approach in a expert case study and a user study with a simulated 7DoF JACO assistive robot arm.
Our results suggest that \algabbr significantly outperforms prior approaches when assisting for unknown intents, maintains high performance in the case of known ones, and successfully learns new intents for better lifelong shared autonomy.

%In Section~\ref{sec:method}, we derive our approach which is based off of prior work on goal assistance \cite{dragan2013blending}, but with added situational confidence that can recognize when none of the robot's hypotheses match the current human behavior \cite{bobu2020quantifying}. Then, in Section~\ref{sec:expert} we examine the performance of our system when assisting an expert user with both known and unknown skills. We show that \algabbr is able to quickly infer the correct goal when goals are all known and quickly relinquish control when the human is attempting a novel skill. Finally, in Section~\ref{sec:userstudy} we run a user study with inexperienced users. 
%Our results show that our method significantly outperforms prior approaches for shared autonomy when assisting for unknown skills, while maintaining high performance in the case of known ones.
%preferred our method to baselines and found \algabbr less frustrating and easier to use \textbf{[add some numbers or other details]}.



% Suppose we have a human and a controllable robot. The human wishes to use the robot to perform some tasks, which may be known or unknown a priori to the robot. We want to improve the assistive capability of the robot by having the robot estimate its confidence in its model of the human's goals. In particular, some questions/objectives are:
% \begin{enumerate}
%     \item Can the robot estimate confidence for pre-programmed goals? (Can the robot evaluate whether the human's behavior is explainable by a goal represented by a pre-programmed value function?)
%     \item Can the robot use its confidence estimates to assist more effectively? (i.e. assist less “aggressively” when it is not confident)
%     \item Can the robot use its confidence estimates to understand when it should attempt to learn new goals?
%     \item What types of goals should the robot learn and how should it learn them, such that it would be able to:
%     \item[a.] Do inference over them in addition to the pre-programmed goals;
%     \item[b.] Assist for them;
%     \item[c.] Estimate confidence for them.
% \end{enumerate}


% \section{RELATED WORK} \label{sec:relatedwork}
% shared control teleoperation



% potential fields approach \cite{aigner1997human}

% Shared autonomy pHIR review paper \cite{losey2018review}. %seems like a nice survey paper. Need to read up and add methods on intent detection and arbitration. the feedback section sounds interesting, but I'm not sure how related that is. Also probably has interesting applications.


% %Talk breifly about applications of shared control. Maybe in intro?
% Shared control has applications to 

% -Handling radioactive waste. \cite{farraj2018hapticshared,goertz1963manipulators}

% Uses haptic-enabled shared control where control algo takes care of some of the degrees of freedom and human controls others \cite{farraj2018hapticshared}

% \cite{goertz1963manipulators}

% -Assisting users to eat or cook


% Learns latent actions via state-conditioned autoencoder that provide low-dimensional human control of high-dimensional robot actuation, but doesn't look at shared autonomy \cite{losey2020latent}.

% -rehabilitation

% \cite{losey2018review}

% -quadrotor control
% Deep reinforcement learning approach \cite{reddy2018shared} --> but even they show that knowing a goal representation drastically improves assistance compared to simply using raw action embeddings.

==> [ICRA'21][Zurek]Situational Confidence Shared Autonomy wbbl/2_method.tex <==
\section{Confidence-Aware Shared Autonomy}
\label{sec:method}

We consider a human teleoperating a dexterous robotic manipulator to perform everyday manipulation tasks.
The robot's goal is to assist the person in accomplishing their desired skill by augmenting or changing their input. %\adremove{ with a semi-autonomous control}.%not sure what combining with semiautonomous means 
While the robot possesses a predefined set of possible intents, the human's desired motion might not be captured by any of them.
We propose that since the robot might not understand the person's intentions, it should reason about how confident it is in its predictions to avoid assisting for the wrong intent.

\subsection{Preliminaries}

Formally, let $\sysstate\in\sset$ be the continuous robot state (e.g. joint angles), and $\action\in\aset$ the continuous robot action (e.g. joint velocity).
The user controls their desired robot configuration by providing continuous inputs $\hinput\in\hset$ via an interface (e.g. GUI, joystick, keyboard commands, etc). These inputs are mapped to robot actions through a \textit{direct teleoperation} function $\mathcal{T} : \hset \rightarrow \aset$. Define a person's trajectory up until time $t$ as the sequence $\traj_{0\to t} = (\sysstate^0, \hinput^0, \hdots, \sysstate^t, \hinput^t)$.

The robot is equipped with a set of known intents $\gset$, one of which may represent the user's desired motion. Each intent is parameterized by a cost function $\cost_\goal$, which may be hand-engineered or learned from demonstrations via IRL~\cite{maxent,Ng2000inverse}. For example, if the intent represents moving to a goal $g$, the cost function can be distance to the goal: $\cost_g(\traj)=\sum_{x\in\traj}\|x-g\|$. If the intent is pouring a cup, the cost can be a neural network with parameters $\psi$, $\cost_\psi$. 
%\adnote{we shold write out something that relates desired motion to the parameter to define and ground what it means to represent skills via cost functions; then give examples: if it's a goal, if it's pouring...}
%In our shared autonomy setup, the robot must combine the user's input with a semi-autonomous control to achieve a common goal. 
Our shared autonomy system does not know the intent a priori, but infers it from the human's inputs. 
Given the user's trajectory so far, $\traj_{0\to t}$, a common strategy is to predict the user's intent $\goal\in\gset$, compute the optimal action for moving accordingly, then augment the user's original input with it~\cite{dragan2013blending}.

However, what if none of the intents match the human's input, i.e., the person is trying to do something the robot does not know about?
We introduce a shared autonomy formalism where the robot reasons about its confidence in its current set of intents' ability to explain the person's input, and uses that confidence for robust assistance. This confidence serves a dual purpose, as the robot can also use it to ask the human to demonstrate 
%(since when you switch to direct control you are getting a first demo)} teach it 
the missing intent.

\subsection{Intent Inference}
\label{sec:skill_inference}

To assist the person, the robot has to first predict which of its known tasks the person is trying to carry out, if any.
To do that, the robot needs a model of how people teleoperate it to achieve a desired motion. 
We assume the Boltzmann noisily-rational decision model~\cite{baker2007goal,von1945theory}:
%
\begin{equation}
    P(\traj \mid \goal, \beta) = \frac{e^{-\beta \cost_{\goal}(\traj)}}{\int_{\bar{\traj}}e^{-\beta \cost_{\goal}(\bar{\traj})} d\bar{\traj}} \enspace ,
    \label{eq:boltzman_trajs}
\end{equation}
%
where the person chooses the trajectory $\traj$ proportional to its exponentiated cost $\cost_\goal$. The parameter $\beta \in [0, \infty)$ controls how much the robot expects to observe human input consistent with the intent $\goal$. Typically, $\beta$ is fixed, recovering the Maximum Entropy IRL observation model~\cite{maxent}, which is what most inference-based shared autonomy methods use~\cite{dragan2013blending,javdani2015shared}.
Inspired by work on confidence-aware human-robot interaction~\cite{fridovich-keil2019confidence,fisac2018probabilistically,bobu2020quantifying}, we instead reinterpret $\beta$ as a measure of the robot's \textit{situational confidence} in its ability to explain human data, given the known intents $\gset$,
and we show how the robot can estimate it in Sec. \ref{sec:confidence_estimation}. 

Given Eq.~\eqref{eq:boltzman_trajs}, if the cost $\cost_\goal$ of intent $\goal$ is additive along the trajectory $\traj$, we have that:
%
\begin{equation}
P(\traj_{0 \to t}\mid \goal, \beta) = e^{-\beta \cost_\goal(\traj_{0 \to t})} \frac{\int_{\bar\traj_{t \to T}} e^{-\beta \cost_\goal(\bar\traj_{t \to T})} }{\int_{\bar\traj_{0 \to T}} e^{-\beta \cost_\goal(\bar\traj_{0 \to T})} }\enspace,
\end{equation} 
%
where $T$ is the duration of the episode. In high-dimensional manipulation spaces, evaluating these integrals is intractable. We follow \cite{dragan2013blending} and approximate them via Laplace's method:
%
\begin{eqnarray}
P(\traj_{0 \to t}\mid \goal, \beta) \approx e^{-\beta \left(\cost_\goal(\traj_{0 \to t}) + \cost_\goal(\traj^*_{t \to T}) - \cost_\goal(\traj^*_{0 \to T})\right)} \nonumber \\
\times \sqrt{\left(\frac{\beta}{2\pi}\right)^{tk}\frac{|\nabla^2 \cost_\goal(\traj^*_{0 \to T})|}{|\nabla^2 \cost_\goal(\traj^*_{t \to T})|}}\enspace,
\label{eq:laplace}
\end{eqnarray}
%
where $k$ is the action dimensionality, and the trajectories $\traj^*_{0 \to T}$ and $\traj^*_{t \to T}$ are optimal with respect to $\cost_\goal$ and can be computed with any off-the-shelf trajectory optimizer\footnote{We use TrajOpt~\cite{trajopt}, based on sequential quadratic programming.}.

Now, given a tractable way to compute the likelihood of the human input, the robot can obtain a posterior over intents:
%
\begin{equation}
    P(\goal \mid \traj_{0 \to t}, \beta) = \frac{P(\traj_{0 \to t}\mid \goal, \beta)}{\sum_{\goal' \in \gset} P(\traj_{0 \to t}|\goal', \beta)},
    \label{eq:goal_inference}
\end{equation}
%
assuming $P(\goal\mid\beta)=P(\goal)$ and a uniform prior over intents. 

Prior inference-based shared autonomy work~\cite{dragan2013blending,javdani2015shared} typically assumes $\beta=1$.
%Note that the above formulation we propose is a generalization of prior inference-based shared autonomy work~\cite{dragan2013blending,javdani2015shared}, which assume $\beta=1$.\adnote{none of this is new, and calling it generalization because you have a beta in front is too strong; state upfront that we follow prior work and recap it here for completeness}
%So far, we have pretended that $\beta$ is given, which is true for typical inference-based shared autonomy methods~\cite{dragan2013blending,javdani2015shared} that simply set $\beta=1$. 
We show that the robot should not be restricted by such an assumption and it, in fact, benefits from estimating $\hat\beta$ and reinterpreting it as a confidence.

%To do so, the robot must predict how the person would like it to execute that skill. 

%We assume there is a set of known skills $\mathcal{S}$ that the robot seeks to assist the human in accomplishing. 
%We have a human teleoperating a robot, the human may be attemting either a known or unknown skill. The goal of the robot is to maximize the performance of the human with respect to the humans true desired skill/goal.  \textbf{TODO: add math notation and make this more precise}
   

\iffalse

\subsection{Goal representation for pre-programmed goals}

The pre-programmed goals are currently all of the form ``move to some goal position g". Letting g be a parameter, any goal of this type can be represented by the robot as a cost function:
\begin{equation}
    C_g(s) = dist(s, g),
\end{equation} with a penalty for the magnitude of the robot's velocity. 
% Alternatively one can also use 
% \begin{equation}
%     V_g(s) = \sum \textrm{squared velocities along shortest path to }g.
% \end{equation}

\subsection{Goal Inference}

We assume that the user is noisily optimal, so they take action $a$ with probability 
\begin{equation}
P(a|s) \propto e^{\beta Q(s, a)},
\end{equation}
where $Q = Q_g$ is the Q-function for the current goal, and $\beta$ controls the strength of the influence of this goal and is related to the confidence estimation. 

Thus human actions give evidence about their true goal (as well as the $\beta$ parameter, if you choose to allow it to have multiple possible values), so by Bayes's Rule 
\begin{equation}
    P(g|a, s) = \frac{P(a|g, s)}{\sum_{g' \in G} P(a|g', s)},
\end{equation}
where we have cancelled the $P(g|s)$ terms as we assume them to be uniformly distributed.
However, to use this, we need to actually find $P(a|g, s)$ which involves two intractable integrals (let $\xi_{t \to t'}$ denote a sequence of states and actions from time $t$ to time $t'$):
\begin{equation}
P(\xi_{t \to t'}| g, \beta) = e^{-\beta C_g(\xi_{t \to t'})} \frac{\int_{\xi'_{t' \to T}} e^{-\beta C_g(\xi'_{t' \to T})} }{\int_{\xi'_{t \to T}} e^{-\beta C_g(\xi'_{t \to T})} }.
\end{equation} 
Using the fact that we can compute optimal trajectories with a trajectory optimizer, we follow prior work \cite{dragan2013blending,bobu2020quantifying} and approximate these using the Laplace approximation  to get 
\begin{eqnarray}
P(\xi_{t \to t'}|g, \beta) \approx e^{-\beta \left(C_g(\xi_{t \to t'}) + C_g(\xi^*_{t' \to T}) - C_g(\xi^*_{t \to T})\right)} \nonumber \\
\times \sqrt{\left(\frac{\beta}{2\pi}\right)^{(t'-t)d}\frac{|\nabla^2 C_g(\xi^*_{t \to T})|}{|\nabla^2 C_g(\xi^*_{t' \to T})|}}.
\end{eqnarray}

% \begin{eqnarray}
% P(\xi_{t : t'}|g, \beta) \approx e^{-\beta  \bar{C}_g(\xi_{t:t'}) } \cdot \sqrt{\left(\frac{\beta}{2\pi}\right)^{(t'-t)d} \cdot H_g(t')}.
% \end{eqnarray}
% where $\bar{C}_g(t') = C_g(\xi_{t \to t'}) + C_g(\xi^*_{t' \to T}) - C_g(\xi^*_{t \to T})$
% and $H_g(t') = |\nabla^2 C_g(\xi^*_{t : T})|/|\nabla^2 C_g(\xi^*_{t':T})|$

\fi

\subsection{Confidence Estimation}
\label{sec:confidence_estimation}

In the Boltzmann model in Eq.~\eqref{eq:boltzman_trajs}, we see that $\beta$ determines the variance of the distribution over human trajectories. When $\beta$ is high, the distribution is peaked around those trajectories $\xi$ with the lowest cost $\cost_\goal$; in contrast, a low $\beta$ makes all trajectories equally likely. We can, thus, reinterpret $\beta$ to take a useful meaning in shared autonomy: given an intent, $\beta$ controls how well that intent's cost explains the user's input. A high $\beta$ for an intent $\goal$ indicates that the intent's cost explains the input well and is a good candidate for assistance. A low $\beta$ on all intents suggests that the robot's intent set is insufficient for explaining the person's trajectory.

%\adnote{give first the idea: how might we detect that the human's input is for a new task/skill that we're missing? if the human's input is irrational for all of these cost functions. -> estimate beta}
We can thus estimate $\beta$ and use it for assistance. Using the likelihood function in Eq.~\eqref{eq:laplace}, we write the $\beta$ posterior
%
\begin{equation}
    P(\beta \mid \traj_{0 \to t}, \goal) = \frac{P(\traj_{0 \to t}\mid \goal, \beta)P(\beta)}{\int_{\bar\beta} P(\traj_{0 \to t}|\goal, \bar\beta)P(\beta)d\bar\beta}.
\end{equation}
%
%While we could handle $\beta$ the same way that we handle goals and follow the blueprint of the above section to infer $\beta$, the expression we get after taking the Laplace approximation decays very rapidly for the wrong $\beta$, so it works to just use the MLE estimate of $\beta$, 
If we assume a uniform prior $P(\beta)$, we may compute an estimate of the confidence parameter $\beta$ per intent $\goal$ via a maximum likelihood estimate:
%
\begin{equation}\label{eq:max_lik_beta}
     \hat\beta_\goal=\arg\max_{\bar\beta} e^{-\bar\beta \left(\cost_\goal(\traj_{0 \to t}) + \cost_\goal(\traj^*_{t \to T}) - \cost_\goal(\traj^*_{0 \to T})\right)}
 \left(\frac{\bar\beta}{2\pi}\right)^{\frac{tk}{2}}\enspace,
\end{equation}
%
%\adnote{remind reader what d is (actually i dont even remember it being defined)}
where we drop the Hessians since they don't depend on $\beta$. Setting the derivative of the objective in Eq.~\eqref{eq:max_lik_beta} to zero and solving for $\beta$ yields the following estimate:
%
\begin{equation}\label{eq:beta_mle}
\hat\beta_{\goal}^{MLE} = \frac{tk}{2(\cost_\goal(\traj_{0 \to t}) + \cost_\goal(\traj^*_{t \to T}) - \cost_\goal(\traj^*_{0 \to T})) }\enspace.
\end{equation}
%
Alternatively, we chose to add an exponential prior with parameter $\lambda$, $Exp(\lambda)$, on $\beta$ to obtain a MAP estimate 
%
\begin{equation}\label{eq:beta_map}
    \hat\beta_{\goal}^{MAP} = \frac{tk}{2( \lambda + \cost_\goal(\traj_{0 \to t}) + \cost_\goal(\traj^*_{t \to T}) - \cost_\goal(\traj^*_{0 \to T})) }\enspace.
\end{equation}
%
%\adnote{what's lambda?}
The denominators in equations \ref{eq:beta_mle} and \ref{eq:beta_map} can be interpreted as the ``suboptimality'' of the observed partial trajectory $\traj_{0 \to t}$ compared to the cost of the optimal trajectory for the particular $\goal$, $ \cost_\goal(\traj^*_{0 \to T})$. Note that
$\hat\beta_\goal$ is inversely proportional to the suboptimality divided by the number of time steps $t$ that have passed. 
Intuitively, the user has more chances to be a suboptimal teleoperator as time goes on, so dividing for $t$ corrects for the natural increase in suboptimality over time. 

If this normalized suboptimality is low for an intent $\goal$, then the person is close to a good trajectory for that intent and $\hat\beta_\goal$ will be high. Thus, a high $\hat\beta_\goal$ means that the person's input is well-explained by that intent.
On the other hand, high suboptimality per time means the person is far from good trajectories, so $\goal$'s cost model $\cost_\goal$ does not explain the person's trajectory and $\hat\beta_\goal$ will be low.

%In the next section we discuss how the robot can adapt its assistance based on its confidence $\hat\beta_\goal$.

%Just by checking if the $\beta$ estimates for a particular goal are above or below a threshold, the robot can tell whether the user was following that cost function or not, and so if all goals have low $\beta$ estimates, the robot should try to learn a new goal.

\comment{
\begin{figure*}
\centering
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=\textwidth,clip=false]{figures/ExpertKnownGoalPybullet.png}
\end{subfigure}
\centering
\begin{subfigure}{.7\textwidth}
  \centering
  \includegraphics[width=\textwidth,clip=false]{figures/ExpertKnownGoalRow.pdf}
\end{subfigure}
\centering
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=\textwidth,clip=false]{figures/ExpertUnknownGoalPybullet.png}
\end{subfigure}
\centering
\begin{subfigure}{.7\textwidth}
  \centering
  \includegraphics[width=\textwidth,clip=false]{figures/ExpertUnknownGoalRow.pdf}
\end{subfigure}
\caption{TODO.\abnote{update firgure to include pouring,write caption, update text referring to the figure}\adnote{add labels maybe on the left hand side in vertical text to say know goal, unknown goal, unknown skill (pouring)}}
\label{fig:case_study}
\end{figure*}
}

\begin{figure*}
%\vspace*{-0.5cm}
\centering
\includegraphics[width=0.9\textwidth]{figures/ExpertStudyFigure.pdf}
\caption{Expert case study results. For each of three manipulation tasks, we compute confidence estimates before learning and, for the misspecified tasks (middle, bottom), we recompute the confidence estimates after learning. We also plot the strength of assistance before and after learning and compare to a policy blending baseline~\cite{dragan2013blending}.}
\label{fig:case_study}
\vspace*{-0.5cm}
\end{figure*}


\subsection{Confidence-based Arbitration}

\comment{
Armed with an estimate of the confidence $\hat\beta_\goal$ for every intent $\goal\in\gset$, the robot can now predict the most likely intent $\goal^* = \arg\max_{\goal\in\gset} P(\goal\mid \traj_{0\to t},\hat\beta_\goal)$ using Eq. \eqref{eq:goal_inference}. 
To assist for it, the robot reasons about how the person would like the task to be executed by computing an optimal trajectory $\traj^*=\arg\min_\traj\sum_{\sysstate\in\traj}\cost_\goal^*(\sysstate)$, and chooses the first action $\action^*$.%\adnote{I think this part should be an equation and shold come up when we introduce the skills as costs} %Here we optimize $\cost_{\goal^*}$, although this cost function does not have to be the same as for teleoperation. 

Now, given the robot's predicted next action $\action^*$ and the human's original action $\hinput^t$, the shared autonomy system has to combine them to best assist the human.
One way to so is by using the ``policy blending'' style of assistance~\cite{dragan2013blending}, which combines $\action^*$ and $\mathcal{T}(\hinput^t)$ using a blending parameter $\alpha\in[0,1]$, resulting in the robot action $\action^t = \alpha \mathcal{T}(\hinput^t) + (1-\alpha) \action^*$.
}

Armed with a confidence estimate $\hat\beta_\goal$ for every $\goal\in\gset$, the robot can predict the most likely one $\goal^* = \arg\max_{\goal\in\gset} P(\goal\mid \traj_{0\to t},\hat\beta_\goal)$ using Eq. \eqref{eq:goal_inference}.
From here, one natural style of assistance is ``policy blending'' ~\cite{dragan2013blending}.
First the robot computes an optimal trajectory under the most likely intent, $\traj^*=\arg\min_\traj\sum_{\sysstate\in\traj}\cost_\goal^*(\sysstate)$, the first action of which is $\action^*$. %\adnote{I think this part should be an equation and shold come up when we introduce the skills as costs} %Here we optimize $\cost_{\goal^*}$, although this cost function does not have to be the same as for teleoperation.
Then the robot combines $\action^*$ and $\mathcal{T}(\hinput^t)$ using a blending parameter $\alpha\in[0,1]$, resulting in the robot action $\action^t = \alpha \mathcal{T}(\hinput^t) + (1-\alpha) \action^*$. We also refer to $\alpha$ as the human's control authority.

Prior work proposes different ways to arbitrate between the robot and human actions by choosing $\alpha$ proportional to the robot's distance to the goal or to the probability of the most likely goal \cite{dragan2013blending}. %\adnote{I actually did it also based on the probability of the most likely goal, i.e. confidence; did you implement it with distance?}. 
%Apart from not being applicable to skills other than going to goals, this heuristic choice of $\alpha$ can fail dramatically in the misspecified situations we are interested in tackling. 
However, when using the probability $P(\goal^*\mid\traj)$, $\goal^*$ might look much better than the other intents, resulting in the robot wrongly assisting for $\goal^*$. Distance-based arbitration ignores the full history of the user's input and can only accommodate simple intents.
%For example, in Fig. \ref{fig:front_fig}, the person tries to go to the orange goal, but because the robot does not know about it, this method incorrectly assists for the closest known goal, the red one.%\adnote{need to explain why that's better than using the prboability of that skill g; it's actually pretty subtle and it'd be good to have an example where you end up with a problem from doing that}

Instead, we propose that the robot should use its confidence in the most likely intent, $\hat\beta_{\goal^*}$, estimated according to Sec. \ref{sec:confidence_estimation}, to control the strength of its arbitration: %$\alpha=\min(1, \frac{1}{\hat\beta_{\goal^*}})$.
%As such, the strength of the robot's influence can increase as the robot is more confident that the observed human inputs are explained by the particular goal. 
%
\begin{equation}
    \action^t = \min(1, 1/\hat\beta_{\goal^*}) \mathcal{T}(\hinput^t) + (1-\min(1, 1/\hat\beta_{\goal^*})) \action^*
\end{equation}
%
When $\hat\beta_{\goal^*}$ is high, i.e. the robot is confident that the predicted intent $\goal^*$ can explain the person's input, $\alpha$ is low, giving the robot more influence through its action $\action^*$. When $\hat\beta_{\goal^*}$ is low, i.e. not even the most likely intent explains the person's input, $\alpha$ increases, giving the person's action $\hinput^t$ more authority.
%\adnote{add an equation on arbitration with beta to make it clear}
%We are using the “policy blending” style of assistance, which combines the human input $a$ with the optimal input (according to the inferred goal) $a^*$ using a blending parameter $\alpha$, so the robot takes action $\alpha a + (1-\alpha) a^*$. 
%This procedure is structurally the same as techniques from~\cite{dragan2013blending}, except that for $\alpha$ we use a function of $\beta$ so that the strength of the robot's influence can increase as the robot is more confident that the observed human inputs are explained by the particular goal. We compute the optimal input according to the inferred goal, $a^*$, by taking the same value function that we were using in our user model and passing it as the objective into a trajectory optimizer. 

\subsection{Using Confidence for Lifelong Learning}
\label{sec:IRL}
%\adnote{write math for how learning (IRL) works to learn a new skill, dont just explain in words}

Estimating the confidence $\hat\beta_{\goal}$ also lets the robot detect \textit{misspecification} in $\gset$: if all estimated $\hat\beta_{\goal}$ for $\goal\in\gset$ are below a threshold $\epsilon$, the robot is missing the person's intent.

Once the robot has identified that its intent set is misspecified, it should ask the person to teach it. 
We represent the missing intent $\goal_\phi$ as a neural network cost parameterized by $\phi$ and learn it via deep maximum entropy IRL~\cite{finn2016guided}.
The gradient of the IRL objective with respect to the cost parameters $\phi$ can be estimated by: $\nabla_{\phi}\mathcal{L} \!\approx\! \frac{1}{|\mathcal{D}^*|}\sum_{\tau \in \mathcal{D}^*} \!\!\nabla_{\phi}\cost_{\phi}(\tau) \!-\! \frac{1}{|\mathcal{D}^{\phi}|}\sum_{\tau \in \mathcal{D}^{\phi}}\!\! \nabla_{\phi}\cost_{\phi}(\tau)$. $\mathcal{D^*}$ are (noisy) demonstrations of the person executing the desired missing intent via direct teleoperation, and
$\mathcal{D}^{\phi}$ are trajectories sampled from the $\cost_\phi$ induced near the optimal policy.%, which we obtain using TrajOpt~\cite{trajopt}.
%With just a few (noisy) demonstrations $\mathcal{D^*}$ of the person executing the desired missing skill via direct teleoperation, the robot can learn an expressive cost function. 


Once we have a new intent $\goal_\phi$, the robot updates its intent set $\gset \gets \gset \cup \goal_\phi$. The next time the person needs assistance, the robot can perform confidence estimation, goal inference, and arbitration as before, using the new library of intents. While the complexity scales linearly with $| \gset |$, planning can be parallelized across each intent.


Learned rewards fit naturally into our framework, allowing for a simple way to compare against the known intents. However, one could imagine adapting our method to the many other ways to learn an intent, from imitation learning~\cite{ho2016GAIL,reddy2020sqil}, to dynamic movement primitives~\cite{paraschos2013PMP}. For instance, if we parameterize intents via policies, we can derive a similar confidence metric based on probabilities of observed human actions under a stochastic policy, rather than costs.

%Since the above techniques for inference and assistance work as long as we have a cost function for the goal, we learn value functions via deep maxent IRL~\cite{finn2016guided}. We then replace the pre-programmed cost function from the above expressions for intent inference and confidence estimation with our learned cost function, and likewise for assistance we can plug this learned cost function into the objective of the trajectory optimizer.



==> [ICRA'21][Zurek]Situational Confidence Shared Autonomy wbbl/3_casestudy.tex <==
\section{Expert Case Study}
\label{sec:expert}

\begin{figure}
\includegraphics[width=\linewidth]{figures/AlphaMethods.pdf}
\centering
\caption{Analysis of arbitration methods. After tracking an optimal trajectory for the Unknown Goal task, we show the robot's belief and confidence estimates for each known goal (left), as well as the $\alpha$ values under the distance, belief, and confidence-based arbitration schemes (right).}
\label{fig:alpha_methods}
\vspace*{-0.5cm}
\end{figure}

In this section, we introduce three manipulation tasks and use expert data to analyze confidence estimation and assistance.
We later put \algabbr's assistive capacity to test with non-experts in a user study in Sec. \ref{sec:userstudy}.

\subsection{Experimental Setting}
%Introduce the three different scenarios. Robot arm setup. Goals, etc.
%\textbf{TODO: set the stage for each experiment with an image? and a description of the scenario and what it tests.}

We conduct our experiments on the simulated 7-DoF JACO arm shown in Fig. \ref{fig:case_study}. We use the pybullet interface~\cite{coumans2019} and teleoperate the robot via keypresses. We map 6 keys to bi-directional $xyz$ movements of the robot's end-effector, and 2 keys for rotating it in both directions. We performed inference and confidence estimation twice per second.

We test \algabbr on 3 different tasks. 
%In the first, deemed \textit{Known Goal}, we control for the situation where there is no misspecification: 
In the \textit{Known Goal} task, we control for the well-specified setting: 
%so the robot's set $\gset$ contains the human's skill. 
the robot must assist the user to move to the known green goal location in Fig. \ref{fig:case_study}. 
In the other tasks, we test CASA's efficacy in the case of misspecification, where the user's desired intent is initially missing from the robot's known set $\gset$.
%In the second task, \textit{Unknown Goal}, the person teleoperates the robot to the red goal which is unknown by the robot. Finally, in the third task, \textit{Unknown Skill}, the person tries a more complicated intent which involves pouring the contents of the cup at a goal location unknown to the robot. 
In the second task, \textit{Unknown Goal}, the person teleoperates the robot to the red goal which is unknown to the robot. Finally, in the third and most complicated task, \textit{Unknown Skill}, the person tries to pour the cup contents at an unknown goal location. 

For the Unknown Goal and Unknown Skill tasks, we first run \algabbr before being exposed to the new intent (\algabbr \textit{before learning}). Detecting low confidence, the robot then asks for demonstrations and learns the missing intents via deep maximum entropy IRL as discussed in Sec. \ref{sec:IRL}. We then run teleoperation with \algabbr \textit{after learning}, to assess the quality of robot assistance after learning the new intent.

\begin{figure*}
%\vspace*{-0.5cm}
\centering
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=\textwidth,clip=false]{figures/UserStudyError.pdf}
\end{subfigure}
\centering
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=\textwidth,clip=false]{figures/UserStudyEfficiencyCost.pdf}
\end{subfigure}
\centering
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=\textwidth]{figures/UserStudyRelativeEffort.pdf}
\end{subfigure}
\caption{Our user study objective metrics. For every task, we measured error with respect to an intended trajectory (left), smoothness of the executed trajectory (middle), and effort relative to direct teleoperation (right).}
\label{fig:study_objective}
\vspace*{-0.5cm}
\end{figure*}

\subsection{Arbitration Method Comparison}
We compare \algabbr to a policy blending assistance (PBA) baseline \cite{dragan2013blending} that assumes $\beta=1$ for all intents. PBA arbitrates with the distance $d_{\goal^*}$ to the predicted goal: $\alpha = \min(1, d_{\goal^*}/D)$, with $D$ some threshold past which the robot does not assist. More sophisticated arbitration schemes use $P(\goal^* \mid \traj)$ or the full distribution $P(\goal \mid \traj)$, but they are much less robust to task misspecification. This is because when the user teleoperates for an unknown intent, $P(\traj \mid \goal)$ will be low for all known $\goal \in \gset$; however, forming $P(\goal \mid \traj)$ requires normalizing over all known intents, after which $P(\goal^* \mid \traj)$ can still be high unless the user happened to operate in a way that appears equally unlikely under all known intents.

We analyzed this phenomenon by tracking a reference trajectory for the Unknown Goal task which moves optimally towards the unknown goal (see Fig.~\ref{fig:case_study} for the task layout). We compared the performances of the distance and confidence arbitration methods, as well as a belief-based method which sets $\alpha = (P(\goal^* \mid \traj)|\gset| - 1)/(|\gset|-1)$ (chosen so that $\alpha= 0$ when $P(\goal^* \mid \traj) = 1/|\gset|$, $\alpha= 1$ when $P(\goal^* \mid \traj) = 1$). In Fig.~\ref{fig:alpha_methods}, the confidence in each goal stays low enough that the robot would have left the user in full control; meanwhile, the relatively higher likelihood of one goal causes the belief $P(\goal^* \mid \traj)$ to quickly go to $1$ and thus set the user's control authority to $0$ under the belief-based arbitration scheme.

We examined one belief-based arbitration method here, but since $P(\goal^* \mid \traj)$ rapidly goes to $1$, any other arbitration that is a function of the belief $P(\goal \mid \traj)$ would similarly try to assist for the wrong goal, motivating our choice of the simpler but more robust distance-based arbitration baseline. %In the user study, we also compare \algabbr to direct teleoperation with no assistance (NA), but this comparison is unnecessary here because we want to analyze how known and new intents affect $\alpha$. 

\subsection{Well-specified Tasks}

Fig. \ref{fig:case_study} (top) showcases the results of our experiment for the Known Goal task. Looking at the confidence plot, we see that $\hat\beta_\goal$ increases with time for the correct green goal, while it remains low for the alternate known purple goal. In the arbitration plot, as $\hat\beta_{\goal^*}$ increases, $\alpha$ gradually decreases, reflecting that the robot takes more control authority only as it becomes more confident that the person's intent is indeed $\goal^*$. Similarly, since there is no misspecification, PBA arbitration steadily decreases the human's contribution to the final control. Both methods result in smooth trajectories which go to the correct goal location. 

\subsection{Misspecified Tasks}


Our approach distinguishes itself in how it handles misspecified tasks. During the Unknown Goal task, in Fig. \ref{fig:case_study} (middle), \algabbr before learning estimates low $\hat\beta_\goal$ for both goals, since neither goal explains the person's motion moving towards the red goal. The estimated $\hat\beta_\goal$ is slightly higher for the green goal than for the purple one because it is closer to the user's input; however, neither are high enough to warrant an arbitration $\alpha$ below $1$, and thus the robot receives no control. In Fig. \ref{fig:case_study} (bottom), we observe almost identical behavior before learning for the Unknown Skill task: the known intents do not match the user's behavior, and thus the user is given full control authority and completes the task.

This contrasts PBA, which, for both Unknown Goal and Unknown Skill, predicts the green goal as the intent. Since in both cases the user's desired trajectory passes near the green goal, PBA erroneously takes control and moves the user towards it, requiring the human to counteract the robot's controls to try to accomplish the task.

In the middle plots for each of the misspecified tasks, we observe for \algabbr after learning, the newly-learned intents receive confidence estimates which increase as the robot is able to observe the user, and thus \algabbr contributes more to the control as it becomes confident.


%In the second plot, we see that \algabbr after learning successfully identifies going to the red goal location as the person's intended skill, while keeping $\hat\beta_\goal$ low for the other goals. As reflected by the arbitration plot, since it is confident in its predicted skill $\goal^*$, the robot gradually contributes more to the final control.

%Meanwhile, PBA predicts the green goal as the intended skill and erroneously forces the human to go there, requiring the human to counteract the robot's controls.
%Since PBA's arbitration confidence is based on distance from the predicted goal, the robot's influence is stronger with time but not for the right skill. The result is that with CASA, the robot detects that its skill set is misspecified and relinquishes control to the human, learns what it does not know, then becomes helpful in assisting the person afterwards. With PBA, the robot is wrongly confident in its prediction, hindering the person, and, even worse, not even helping them reach the right goal.

\begin{figure*}
%\vspace*{-0.5cm}
\centering
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=\textwidth,clip=false]{figures/UserStudy_Subjective1.pdf}
\end{subfigure}
\centering
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=\textwidth,clip=false]{figures/UserStudy_Subjective2.pdf}
\end{subfigure}
\centering
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=\textwidth]{figures/UserStudy_Subjective3.pdf}
\end{subfigure}
\caption{Subjective user study results. When there is no misspecification (left), our method is not inferior to PBA, whereas when there is misspecification (center, right), the participants prefer our method after learning a new intent.}
\label{fig:likert}
\vspace*{-0.5cm}
\end{figure*}

==> [ICRA'21][Zurek]Situational Confidence Shared Autonomy wbbl/4_expertstudy.tex <==
\section{User Study}
\label{sec:userstudy}

%\textbf{TODO: Show results from inexperienced users. Focus on task performance for our method as opposed to other methods and user qualitative preferences. Report statistics for different methods.}

%In Sec. \ref{sec:expert}, we analyzed how \algabbr estimates confidence and assists for known and novel tasks, before and after learning. 
We now present the results of our user study, testing how well our method can assist non-expert users.

\subsection{Experimental Design}

Due to the COVID-19 pandemic, we were unable to perform an in-person user study with a physical robot. Instead, as described in Sec. \ref{sec:expert}, we replicated our lab set-up in a pybullet simulator~\cite{coumans2019} in which users can teleoperate a 7 DoF JACO robotic arm using keyboard inputs (Fig. \ref{fig:case_study}). 

We split the study into four phases: (1) familiarization, (2) no misspecification, (3) misspecification before learning, and (4) misspecification after learning. First, we introduce the user to the simulation interface by asking them to perform a familiarization task. In the next phase, we tested the Known Goal task. In the third phase, we tested the two misspecified tasks, Unknown Goal and Unknown Skill, then asked participants to provide 5 demonstrations for each intent. Finally, in the fourth phase, we retested the misspecified tasks using cost functions learned from the demonstrations.

\textbf{Independent Variables:} For each experiment, we manipulate the \textit{assistance method} with three levels: no assistance (NA), policy blending assistance (PBA) \cite{dragan2013blending}, and \algname (\algabbr). For Unknown Goal and Unknown Skill, we compared our method before and after learning new intents against the NA and PBA baselines. 

\textbf{Dependent Measures:} 
Before each task, we displayed an exemplary reference trajectory to help participants understand their objective.
%We also instructed participants to perform the task with as few key presses as needed, to showcase each assistance method.
As such, for our objective metrics, we measured 
\textit{Error} as the sum of squared differences between the intended and executed trajectories,
\textit{Efficiency Cost} as the sum of squared velocities across the executed trajectory,
and \textit{Effort} as the number of keys pressed.
To assess the users' interaction experience, we administered a subjective 7-point Likert scale survey, asking the participants three questions: (1) if they felt the robot understood how they wanted the task done, (2) if the robot made the interaction more effortless, and (3) if the assistance provided was useful.

\noindent\textbf{Participants:}
We used a within-subjects design and counterbalanced the order of the assistance methods.
We recruited 11 users (10 male, aged 20-30) from the campus community, most of whom had technical background.%, but no prior experience with the simulator.

\noindent\textbf{Hypotheses:}

\noindent\textbf{H1:} If there is no misspecification, assisting with \algabbr is not inferior to assisting with PBA, and is superior to NA.

\noindent\textbf{H2:} If there is misspecification, assisting with \algabbr before learning is more accurate, efficient, and effortless than with PBA and not inferior to NA.

\noindent\textbf{H3:} If there is misspecification, assisting with \algabbr after learning is more accurate, efficient, and effortless than NA.

\noindent\textbf{H4:} If there is misspecification, participants will believe the robot understood what they want, feel less interaction effort, and find the assistance more useful with \algabbr after learning than with any other baseline.

\subsection{Analysis}

\noindent\textbf{Objective.}
Fig. \ref{fig:study_objective} summarizes our main findings. For Known Goal, which is well-specified, CASA does no worse than PBA and better that NA in terms of relative effort and error. 
We confirmed this by running an ANOVA, finding a significant main effect for the method ($F(2,30) = 104.93, p < .0001$ for effort; $F(2,30) = 8.93, p = .0009$ for error). In post-hoc testing, a Tukey HSD test revealed that CASA is significantly better than NA ($p < .0001$ for effort, $p = .0013$ for error). 
We also performed a non-inferiority test~\cite{lesaffre2008noninferiority}, and obtained that CASA is non-inferior to PBA within a margin of $0.065$ for effort, $0.025$ for efficiency, and $0.26$ for error. 
These findings are in line with H1 and were expected, since the robot should have no problem handling known intents.

For the two misspecified tasks, we first ran an ANOVA with the method (CASA before learning, NA, and PBA) as a factor, and the task as a covariate, and found a significant main effect ($F(2,62)=11.8255, p<.0001$ for effort; $F(2,62)=6.119, p=.0038$ for error). A Tukey HSD revealed that CASA is significantly better than PBA ($p=.0005$ for effort, $p=.005$ for error). We also ran a non-inferiority test, and obtained that CASA is non-inferior to NA within a margin of $0.035$ for effort, $0.02$ for efficiency, and $1.4$ for error for Unknown Goal, and $0.03$ for effort, $0.09$ for efficiency, and $4.5$ for error for Unknown Skill.
For both unknown tasks, CASA before learning is essentially indistinguishable from NA since a low $\hat\beta_{\goal^*}$ would make the robot rely on direct teleoperation.
Both the figure and our statistical tests confirm H2, which speaks for the consequences of confidently assisting for the wrong intent.

For efficiency cost, we did not find an effect, possibly because Fig.~\ref{fig:study_objective} shows that PBA is more efficient for the Unknown Skill task than other methods. 
Anecdotally, PBA forced users to an incorrect goal thus preventing them from pouring, which explains the lower efficiency cost.
By having a high arbitration for the wrong intent, PBA can cause a smooth trajectory, since it lowers the control authority of the possibly-noisy human inputs. However, this trajectory does not accomplish the task. When running an ANOVA for each of the tasks separately, we found a significant main effect for the method for Unknown Goal ($F(2,30)=9.66, p=.0006$), and a post-hoc Tukey HSD revealed CASA is significantly better than PBA ($p=.0032$), further confirming H2.

Lastly, we looked at the performance with CASA after learning the new intents.
For Unknown Goal, a simple task, the figure shows that CASA after learning doesn't improve efficiency and error, but it does reduce relative effort when compared to NA. 
For Unknown Skill, a more complex task, CASA after learning outperforms NA. This is confirmed by an ANOVA with the method (NA, CASA after learning) as the factor, where we found a significant main effect ($F(1,41)=53.60, p<.0001$ for effort; $F(1,641)=8.6184, p=.0054$ for efficiency cost), supporting H3.

\noindent\textbf{Subjective.}
We show the average Likert survey scores for each task in Fig. \ref{fig:likert}. In line with H1, for the Known Goal task, users thought the robot under both PBA and \algabbr had a good understanding of how they wanted the task to be done, made the interaction more effortless, and provided useful assistance. The results are in stark contrast to NA, which scores low on all those metrics. For Unknown Goal and Unknown Skill, all methods fare poorly on all questions except for CASA after learning, supporting H4.

==> [ICRA'21][Zurek]Situational Confidence Shared Autonomy wbbl/5_discussion.tex <==
\section{Conclusion}
\label{sec:discussion}

In this paper, we formalized a confidence-aware shared autonomy process where the robot can adjust its assistance based on how confident it is in its prediction of the human intent. We introduced an approximate solution for estimating this confidence, and demonstrated its effectiveness in adjusting arbitration when the robot's intent set is misspecified and enabling continual learning of new intents.


While our confidence estimates tolerated some degree of suboptimal user control, an extremely noisy operator attempting a known intent might instead appear to be performing a novel intent. Moreover, due to COVID, we ran our experiments in a simulator, which does not replicate the difficulty inherent in teleoperating a real manipulator via a joystick interface.
%In fact, our user study participants found keyboard control satisfactory in our setup.
Despite these limitations, we are encouraged to see robots have a more principled and robust way to arbitrate shared autonomy, as well as decide when they need to learn more to be better teammates.
We look forward to applications of our confidence-based ideas beyond manipulation robots, to semi-autonomous vehicles, quadcopter control, or any other shared autonomy scenarios.% where assisting people with confidence might be beneficial.

==> [ICRA'21][Zurek]Situational Confidence Shared Autonomy wbbl/macros.tex <==
% For state-related stuff
\newcommand{\sysstate}{x}
\newcommand{\action}{u}
\newcommand{\hinput}{a}
\newcommand{\goal}{\ensuremath{\theta}}

% For sets
\newcommand{\aset}{\ensuremath{\mathcal{U}}}
\newcommand{\sset}{\ensuremath{\mathcal{X}}}
\newcommand{\gset}{\ensuremath{\Theta}}
\newcommand{\hset}{\ensuremath{\mathcal{A}}}

% For cost function stuff
\newcommand{\cost}{C}
\newcommand{\traj}{\ensuremath{\xi}}

